Potentials of Green Coding -- Findings and Recommendations for Industry, Education and Science -- Extended Paper

Progressing digitalization and increasing demand and use of software cause rises in energy- and resource consumption from information and communication technologies (ICT). This raises the issue of sustainability in ICT, which increasingly includes the sustainability of the software products themselves and the art of creating sustainable software. To this end, we conducted an analysis to gather and present existing literature on three research questions relating to the production of ecologically sustainable software ("Green Coding") and to provide orientation for stakeholders approaching the subject. We compile the approaches to Green Coding and Green Software Engineering (GSE) that have been published since 2010. Furthermore, we considered ways to integrate the findings into existing industrial processes and higher education curricula to influence future development in an environmentally friendly way.

==> Tables/Search_Strings_Results.tex <==
%\begin{table}[htp]
  \begin{longtable}[H!]{|m {0.2\textwidth} |m {0.2\textwidth}|m {0.1\textwidth}|m {0.1\textwidth}|m {0.1\textwidth}|}
  \label{tab:Seach_Strings}
  \small
  \hline
  \textbf{\raggedright Search String} & 
  \textbf{\raggedright Purpose} & 
  \textbf{\raggedright Google Scholar Results} & \textbf{\raggedright ACM DL Results} & 
  \textbf{\raggedright dblp \break Results} \\
  \hline 
Implementing green coding in software development &
To find information and guidance on integrating environmentally responsible practices into software development processes.& 
about \break  17800 &  
372.203 & 
0 \\ \hline 

How to integrate sustainability in software development&
To learn the steps and best practices for making software development more sustainable.&
about \break 14.900 &
384.522 & 
0   \\ \hline

Steps to a greener software development process& 
To identify the steps that already exist for the integration of green coding into existing software development processes                               & about \break 17.800  & 
384.522 & 
0 \\ \hline

Best practices for implementing green coding in software engineering&
To identify the steps that already exist for the integration of green coding into existing software engineering processes&
about \break 16.300 & 
378.197 & 
0  \\ \hline

Strategies for implementing sustainable software development&
To identify the actual strategies for sustainable software development. &
about \break 17.800 & 
373.671 & 
0 \\ \hline

(green coding | green computing | green software engineering | sustainable software engineering) AND (practices | recommendations | techniques) &
Searching for concrete measures and guidelines  &
about \break 47. 400 & 
315 & 
0  \\  \hline

(green coding | green computing | green software engineering | Sustainable Software Engineering) AND (practices | challenges | review) &
Searching for existing reviews, summary sources, and research gaps &
about \break 20.100 & 
314 & 
0  \\  \hline

( green coding | green computing | green software engineering | Sustainable Software Engineering) AND ( case stud* | implement* ) & Searching for implementations of or case studies on the usage of green coding practices &
about  \break 17.800 &
317 &
0\\  \hline

(green coding | green computing | green software engineering | sustainable software engineering) &
Search string for dblp, as it did not return any results for the search strings including conjunction above &
about \break21.900 &
317 &
72\\ 
\hline
\end{longtable}
%\end{table}

==> Tables/Stats_RQ1.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
         \hline
         \textbf{Unique publications} & 18 \\
         \hline
         \textbf{Papers included in final analysis} & 21 \\
         \hline
    \end{tabular}
    \caption{Papers}
    \label{tab:my_label}
\end{table}
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
         \hline
         \textbf{Year} & \textbf{\# of papers published} \\
         \hline
         2010 & 0\\
         \hline
         2011 & 1\\
         \hline
         2012 & 2\\
         \hline
         2013 & 1\\
         \hline
         2014 & 4\\
         \hline
         2015 & 0\\
         \hline
         2016 & 1\\
         \hline
         2017 & 5\\
         \hline
         2018 & 2\\
         \hline
         2019 & 1\\
         \hline
         2020 & 0\\
         \hline
         2021 & 2\\
         \hline
         2022 & 2\\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
